EOS: a Parallel, Self-Adaptive, Multi-Population Evolutionary Algorithm for Constrained Global Optimization

This paper presents the main characteristics of the evolutionary optimization code named EOS, Evolutionary Optimization at Sapienza, and its successful application to challenging, real-world space trajectory optimization problems. EOS is a global optimization algorithm for constrained and unconstrained problems of real-valued variables. It implements a number of improvements to the well-known Differential Evolution (DE) algorithm, namely, a self-adaptation of the control parameters, an epidemic mechanism, a clustering technique, an $\varepsilon$-constrained method to deal with nonlinear constraints, and a synchronous island-model to handle multiple populations in parallel. The results reported prove that EOSis capable of achieving increased performance compared to state-of-the-art single-population self-adaptive DE algorithms when applied to high-dimensional or highly-constrained space trajectory optimization problems.

==> LaTeX_Bibliography_Files/README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> pruningLF.tex <==
The term ``space pruning'' refers to those techniques that aim at reducing the solution space during the search,
focusing the optimization in a smaller area where, in accordance with some criteria, good solutions are expected to be found.

Different solution methods have been proposed in the past \cite{vasile2009hybrid, ghojogh2018tree} that combine branching, that is, the subdivision of the feasible region into smaller subdomains (with some convergence properties) and population-based stochastic algorithms, to search in the subdomains in order to evaluate them, showing higher average performance with respect to a number of stochastic and deterministic methods on the same problems.

The pruning method adopted in \textit{EOS} is based on the \textit{cluster pruning algorithm} developed by ESA's Advanced Concept Team \cite{conway2010spacecraft} to solve Multiple Gravity-Assist (MGA) problems.
The key idea is that in problems like MGA and related space trajectory optimization problems (as MGA-1DSM or multi-rendezvous ones), which are the kind of problems addressed by \textit{EOS}, good solutions are often clustered in small regions instead of
being densely distributed over the whole search space.
So, during the optimization process, it is possible to progressively focus the search around the promising regions identified so far, increasing the quality of the solutions found, but accepting the risk that some possibly better solution may be potentially ruled out.

The \textit{pruning-by-clustering} method implemented in \textit{EOS} works as follows.
Let us suppose that we want to run the selected DE algorithm (with $N_p$ individuals) $N_r$ times for $N_G$ generations each time, and elect as putative optimum of the problem the best solution among the $N_r$ solutions found at the last generation.
Without modifying the total number of functions evaluations $FES = N_r N_G N_p$, it is possible to exploit the solutions found by the $N_r$ runs at given points during the evolution process to efficiently drive the search during the remaining number of generations and reduce the solution space on the base of what has been learned so far during optimization.% and progressively focus the search on on the remaining number of generations

Specifically, the first space pruning is performed after $N_{G, pr}^0$ generations, and, in total, $N_{pr}$ pruning events are performed, spaced by $N_{G, pr} = (N_{G} - N_{G, pr}^0)/N_{pr}$ generations each other.
At the $i$-th pruning event, the best individuals found at generation $N_{G, pr}^0 + i N_{G, pr}$ by the $N_r$ parallel optimization runs are sorted on the basis of their fitness. Then, for any design variable $j \in [1,D]$, the new bounding interval $\left[x_{L, new}^{(j)}, x_{U, new}^{(j)}\right]$ to be used in the next $N_{G, pr}$ generations is recomputed by looking at the extreme values assumed by the $j$-th variable in the first (i.e., the best) $N_{p, pr} = \lfloor \rho_{pr} N_p \rfloor$ individuals, with $\rho_{pr} = \rho_{pr}^0 - i \Delta \rho_{pr}$.
The new variable bounds are:
%Every $N_{G, pr} = 500 \div 1000$ generations, the individuals in the current population are sorted on the basis of their fitness. Then, for any design variable $j \in [1,D]$, the new bounding interval $\left[x_{L, new}^{(j)}, x_{U, new}^{(j)}\right]$ to be used in the next generations is recomputed by looking at the extreme values assumed by the $j$-th variable in the first (i.e., the best) $N_{pr} = \lfloor \rho_{pr} N_p \rfloor$ individuals:
\begin{align}
    x_{L, new}^{(j)} &= \min_{i \in [1, N_{pr}]}{x_i^{(j)}} - 0.5 (1 - \rho_{pr}) \left (x_U^{(j)} - x_L^{(j)} \right ) \\
    x_{U, new}^{(j)} &= \max_{i \in [1, N_{pr}]}{x_i^{(j)}} + 0.5 (1 - \rho_{pr}) \left (x_U^{(j)} - x_L^{(j)} \right )
\end{align}
%$\rho_{pr}$ is decreased by a factor $0.05$ at each pruning event, starting from $\rho_{pr} = 0.25$ and arriving to $\rho_{pr} = 0.05$. 
Obviously, these new bounds are used only if they are still within the old bounds. 
After pruning, the $N_r$ optimization procedures are restarted, re-inizialiting the whole population in the newly defined solution space. Moreover, the $N_{p, pr}$ best individuals found by the previously performed $N_r$ runs are copied in each of the new populations, substituting the worst individuals.
The hyper-parameter values that showed the best performance in EOS are the following: $\rho_{pr}^0 = 0.3$, $\Delta \rho_{pr} = 0.1$, $N_{pr} = 3$ and $N_{G, pr}^0 = 0.4N_G$.

==> sezionePruningOld.tex <==
\section{Space Pruning by Clustering}
\label{sec:pruning}
The term ``space pruning'' refers to those techniques that allow reducing the solution space during search,
focusing the optimization in a smaller area where, in accordance with some criteria, good solutions are expected to be found.

Different solution methods have been proposed in the past \cite{vasile2009hybrid, ghojogh2018tree} that combine branching, that is, the subdivision of the feasible region into smaller subdomains (with some convergence properties) and population-based stochastic algorithms, to search in the subdomains in order to evaluate them, showing higher average performance with respect to a number of stochastic and deterministic methods on the same problems.

The pruning method adopted in \textit{EOS} is based on the \textit{cluster pruning algorithm} developed by ESA's Advanced Concept Team \cite{conway2010spacecraft} to solve Multiple Gravity-Assist (MGA) problems.
The key idea is that in problems like MGA and related space trajectory optimization problems (as MGA-1DSM or multi-rendezvous ones), which are the kind of problems to solve through \textit{EOS}, good solutions are often clustered in small portions of the search space instead of
being densely distributed all over it.
So, during the optimization process, it is possible to progressively focus the search around the promising regions identified so far, increasing the quality of the solutions found, but accepting the risk that some possibly better solution may be potentially ruled out.

The \textit{pruning-by-clustering} method implemented in \textit{EOS} works as follows.
Every $N_{G, pr} = 500 \div 1000$ generations, the individuals in the current population are sorted on the basis of their fitness. Then, for any design variable $j \in [1,D]$, the new bounding interval $\left[x_{L, new}^{(j)}, x_{U, new}^{(j)}\right]$ to be used in the next generations is recomputed by looking at the extreme values assumed by the $j$-th variable in the first (i.e., the best) $N_{pr} = \lfloor \rho_{pr} N_p \rfloor$ individuals:
\begin{align}
    x_{L, new}^{(j)} &= \min_{i \in [1, N_{pr}]}{x_i^{(j)}} - \lambda (1 - \rho_{pr}) \left (x_U^{(j)} - x_L^{(j)} \right ) \\
    x_{U, new}^{(j)} &= \max_{i \in [1, N_{pr}]}{x_i^{(j)}} + \lambda (1 - \rho_{pr}) \left (x_U^{(j)} - x_L^{(j)} \right )
\end{align}
These new bounds are used only if they are still within the old bounds. 
In particular, $\lambda = 0.1 \div 0.5$ and
$\rho_{pr}$ is decreased by a factor $0.05$ at each pruning event, starting from $\rho_{pr} = 0.25$ and arriving to $\rho_{pr} = 0.05$. 
